How BERT-based Cross-Encoders Model Relevance in Information Retrieval?

Cross-encoders are the most effective but also the least efficient models in Information Retrieval. Despite their success, the mechanisms underlying their relevance predictions remain poorly understood, particularly how they process to match queries and documents. This lack of interpretability limits their optimization, can lead to suboptimal retrieval, especially out-of-domain, and raises efficiency concerns for over-parameterized models. To address these challenges, this paper investigates two under-explored aspects of cross-encoder behavior. First, to understand the relevance prediction process, we trace the flow of information at the different stages of the process and between different input segments. We study the nature of the signals that compose this flow and that allow cross-encoders to predict the relevance of a passage to a query. Our work particularly focuses on the matching performed by the cross-encoders between queries and documents. Second, we explore how cross-encoders behave with out-of-domain documents and/or queries. Through a series of interpretability experiments, we evaluate three BERT-based cross-encoder models, varying in size and pre-training strategies, across both in-domain and out-of-domain datasets. Overall, this study both consolidates what is known about how cross-encoders model relevance and extends it by exploring the role of matching signals.

==> images_v2/RQ5/ablations_tab.tex <==
\begin{table*}[h]
\centering
\caption{Evaluation Results}
\label{tab:masks_mice}
\begin{tabular}{rcccccccccccc}
\toprule
Model & DL19 & DL20 & BA & Fi & NFC & NQ & R04 & DL21 & DL22 & T-C & Avg. (ID) & Avg. (OOD) \\
\midrule
 & 51.2 & 47.7 & 52.2 & 23.6 & 32.2 & 21.7 & 44.9 & 44.6 & 26.9 & 59.5 & 49.4 & 38.2 \\
 MonoBERT-large & 71.3 & 68.2 & 47.4 & 32.2 & 33.3 & 34.8 & 45.5 & 63.1 & 48.6 & 62.6 & 69.8 & 45.9 \\
%MiniLM & 73.5 & 67.6 & 50.0 & 31.2 & 33.6 & 35.7 & 46.0 & 65.0 & 49.5 & 65.6 & 70.5 & 47.1 \\
%ModernBERT-150m& 72.4 & 67.8 & 53.2 & 33.6 & 34.2 & 34.8 & 44.9 & 66.2 & 50.7 & 70.1 & 70.1 & 48.5 \\
%ModernBERT-32m& 72.2 & 67.2 & 50.8 & 29.8 & 33.3 & 33.5 & 41.9 & 64.0 & 47.4 & 67.7 & 69.7 & 46.0 \\
%MonoBERT-base & 72.8 & 67.8 & 49.6 & 30.1 & 33.2 & 35.9 & 46.7 & 64.4 & 48.7 & 64.4 & 70.3 & 46.6 \\
Mask 0 MonoBERT-large & 49.1 & 43.5 & 25.3 & 15.7 & 24.8 & 20.2 & 29.6 & 40.4 & 25.4 & 48.1 & 46.3 & 28.7 \\
%Mask 0 MiniLM & 73.0 & 67.3 & 48.5 & 30.1 & 33.5 & 34.9 & 44.2 & 63.4 & 47.4 & 66.6 & 70.2 & 46.1 \\
%Mask 0 ModernBERT-150m& 43.9 & 33.1 & 20.1 & 10.0 & 17.7 & 17.2 & 18.7 & 45.0 & 27.0 & 47.3 & 38.5 & 25.4 \\
%Mask 0 ModernBERT-32m& 49.4 & 43.1 & 29.1 & 11.2 & 19.3 & 18.8 & 22.8 & 47.2 & 31.8 & 53.9 & 46.2 & 29.3 \\
%Mask 0 MonoBERT-base & 71.9 & 66.6 & 48.1 & 29.6 & 33.0 & 35.5 & 45.6 & 62.7 & 49.2 & 63.6 & 69.3 & 45.9 \\
 Mask 1 MonoBERT-large & 24.2 & 15.9 & 18.6 & 6.9 & 15.3 & 7.0 & 16.9 & 24.0 & 14.6 & 46.3 & 20.1 & 18.7 \\
%Mask 1 MiniLM & - & 67.2 & 48.4 & 30.1 & 33.5 & 34.6 & 45.0 & 63.6 & 47.2 & 66.4 & 67.2 & 46.1 \\
%Mask 1 ModernBERT-150m& 72.7 & 62.0 & 51.4 & 29.6 & 33.4 & 31.6 & 40.9 & 63.1 & 46.2 & 67.0 & 67.4 & 45.4 \\
%Mask 1 ModernBERT-32m& 62.8 & 54.6 & 38.8 & 15.7 & 28.4 & 25.5 & 36.0 & 55.3 & 38.1 & 61.2 & 58.7 & 37.4 \\
%Mask 1 MonoBERT-base & 71.5 & 65.9 & 47.5 & 28.6 & 32.9 & 34.2 & 45.1 & 61.3 & 47.7 & 64.1 & 68.7 & 45.2 \\
Mask 2 MonoBERT-large & 19.9 & 15.7 & 13.7 & 4.3 & 14.4 & 5.9 & 16.3 & 26.0 & 13.1 & 45.2 & 17.8 & 17.4 \\
%Mask 2 MiniLM & 62.8 & 58.3 & 32.0 & 21.9 & 31.5 & 25.8 & 38.5 & 53.1 & 39.4 & 59.0 & 60.5 & 37.6 \\
%Mask 2 ModernBERT-150m& 69.2 & 61.7 & 47.1 & 27.3 & 33.2 & 30.3 & 39.2 & 60.3 & 44.4 & 69.7 & 65.5 & 43.9 \\
%Mask 2 ModernBERT-32m& 57.7 & 52.5 & 36.4 & 13.8 & 27.8 & 24.2 & 35.2 & 51.7 & 35.6 & 59.9 & 55.1 & 35.6 \\
%Mask 2 MonoBERT-base & 69.6 & 63.5 & 39.0 & 25.9 & 31.7 & 30.5 & 43.3 & 58.2 & 44.4 & 65.0 & 66.6 & 42.2 \\
\bottomrule
\end{tabular}
\end{table*}

==> images_v2/RQ5/ablations_tab_v2.tex <==
\begin{table*}[h]
\centering
\caption{Evaluation Results}
\label{tab:masks_mice}
\begin{tabular}{rcccccccccccc}
\toprule
Model & DL19 & DL20 & BA & Fi & NFC & NQ & R04 & DL21 & DL22 & T-C & Avg. (ID) & Avg. (OOD) \\
\midrule
 & 51.2 & 47.7 & 52.2 & 23.6 & 32.2 & 21.7 & 44.9 & 44.6 & 26.9 & 59.5 & 49.4 & 38.2 \\
MonoBERT-large & 71.3 & 68.2 & 47.4 & 32.2 & 33.3 & 34.8 & 45.5 & 63.1 & 48.6 & 62.6 & 69.8 & 45.9 \\
MiniLM & 73.5 & 67.6 & 50.0 & 31.2 & 33.6 & 35.7 & 46.0 & 65.0 & 49.5 & 65.6 & 70.5 & 47.1 \\
MonoBERT-base & 72.8 & 67.8 & 49.6 & 30.1 & 33.2 & 35.9 & 46.7 & 64.4 & 48.7 & 64.4 & 70.3 & 46.6 \\
\cmidrule(lr){1-13}
ModernBERT-150m & 72.4 & 67.8 & 53.2 & 33.6 & 34.2 & 34.8 & 44.9 & 66.2 & 50.7 & 70.1 & 70.1 & 48.5 \\
ModernBERT-32m & 72.2 & 67.2 & 50.8 & 29.8 & 33.3 & 33.5 & 41.9 & 64.0 & 47.4 & 67.7 & 69.7 & 46.0 \\
\midrule
Mask 0 MonoBERT-large & 49.1 & 43.5 & 25.3 & 15.7 & 24.8 & 20.2 & 29.6 & 40.4 & 25.4 & 48.1 & 46.3 & 28.7 \\
Mask 0 MiniLM & 73.0 & 67.3 & 48.5 & 30.1 & 33.5 & 34.9 & 44.2 & 63.4 & 47.4 & 66.6 & 70.2 & 46.1 \\
Mask 0 MonoBERT-base & 71.9 & 66.6 & 48.1 & 29.6 & 33.0 & 35.5 & 45.6 & 62.7 & 49.2 & 63.6 & 69.3 & 45.9 \\
\cmidrule(lr){1-13}
Mask 0 ModernBERT-150m & 43.9 & 33.1 & 20.1 & 10.0 & 17.7 & 17.2 & 18.7 & 45.0 & 27.0 & 47.3 & 38.5 & 25.4 \\
Mask 0 ModernBERT-32m & 49.4 & 43.1 & 29.1 & 11.2 & 19.3 & 18.8 & 22.8 & 47.2 & 31.8 & 53.9 & 46.2 & 29.3 \\
\midrule
Mask 1 MonoBERT-large & 24.2 & 15.9 & 18.6 & 6.9 & 15.3 & 7.0 & 16.9 & 24.0 & 14.6 & 46.3 & 20.1 & 18.7 \\
Mask 1 MiniLM & - & 67.2 & 48.4 & 30.1 & 33.5 & 34.6 & 45.0 & 63.6 & 47.2 & 66.4 & 67.2 & 46.1 \\
Mask 1 MonoBERT-base & 71.5 & 65.9 & 47.5 & 28.6 & 32.9 & 34.2 & 45.1 & 61.3 & 47.7 & 64.1 & 68.7 & 45.2 \\
\cmidrule(lr){1-13}
Mask 1 ModernBERT-150m & 72.7 & 62.0 & 51.4 & 29.6 & 33.4 & 31.6 & 40.9 & 63.1 & 46.2 & 67.0 & 67.4 & 45.4 \\
Mask 1 ModernBERT-32m & 62.8 & 54.6 & 38.8 & 15.7 & 28.4 & 25.5 & 36.0 & 55.3 & 38.1 & 61.2 & 58.7 & 37.4 \\
\midrule
Mask 2 MonoBERT-large & 19.9 & 15.7 & 13.7 & 4.3 & 14.4 & 5.9 & 16.3 & 26.0 & 13.1 & 45.2 & 17.8 & 17.4 \\
Mask 2 MiniLM & 62.8 & 58.3 & 32.0 & 21.9 & 31.5 & 25.8 & 38.5 & 53.1 & 39.4 & 59.0 & 60.5 & 37.6 \\
Mask 2 MonoBERT-base & 69.6 & 63.5 & 39.0 & 25.9 & 31.7 & 30.5 & 43.3 & 58.2 & 44.4 & 65.0 & 66.6 & 42.2 \\
\cmidrule(lr){1-13}
Mask 2 ModernBERT-150m & 69.2 & 61.7 & 47.1 & 27.3 & 33.2 & 30.3 & 39.2 & 60.3 & 44.4 & 69.7 & 65.5 & 43.9 \\
Mask 2 ModernBERT-32m & 57.7 & 52.5 & 36.4 & 13.8 & 27.8 & 24.2 & 35.2 & 51.7 & 35.6 & 59.9 & 55.1 & 35.6 \\
\bottomrule
\end{tabular}
\end{table*}
